An Anytime, Scalable and Complete Algorithm for Embedding a Manufacturing Procedure in a Smart Factory

Modern automated factories increasingly run manufacturing procedures using a matrix of programmable machines, such as 3D printers, interconnected by a programmable transport system, such as a fleet of tabletop robots. To embed a manufacturing procedure into a smart factory, an operator must: (a) assign each of its processes to a machine and (b) specify how agents should transport parts between machines. The problem of embedding a manufacturing process into a smart factory is termed the Smart Factory Embedding (SFE) problem. State-of-the-art SFE solvers can only scale to factories containing a couple dozen machines. Modern smart factories, however, may contain hundreds of machines. We fill this hole by introducing the first highly scalable solution to the SFE, TS-ACES, the Traffic System based Anytime Cyclic Embedding Solver. We show that TS-ACES is complete and can scale to SFE instances based on real industrial scenarios with more than a hundred machines.

==> old_text.tex <==
% Old Abstract
modern manufacturing industry. Consequently, modern smart machines typically use flexible, general-purpose machines such a CNC machines. Parts are ferried between machines using a flexible transportation system, a transportation system which makes it easy to adjust the flow of parts through a smart factory. Typically, flexible transportation systems transport parts using a team of agents. To embed a manufacturing procedure into a smart factory, an operator must: (a) assign each of its processes to a machine and (b) specify how agents should transport parts between machines. The problem of embedding a manufacturing process into a smart factory is termed the Smart Factory Embedding (SFE) problem. State-of-the-art solutions to the SFE problem have only been shown to scale to factories containing a dozen machines. Modern smart factories, however, may contain hundreds of machines. We fill this hole by proposing the Traffic System based Anytime Cyclic Embedding Solver (TS-ACES), the first highly scalable solution to the SFE. TS-ACES exploits the following observation: most smart factories coordinate agents using a traffic system. TS-ACES uses a MILP to compute a traffic system based embedding, an embedding which specifies, at a high level, how agents should move through the traffic system. It then uses this embedding to compute concrete instructions for each agent. We show that TS-ACES is complete. We evaluate TS-ACES and show that it can scale to SFE instances based on real industrial scenarios with more than a hundred machines.

% Old Update Cargo
\begin{algorithm}[t]
\small
\caption{\updateCargo{}($M, A, t, \T{}, \agentAtM{}, \agClM{}, \agTkM{}, \pkM{}', \dpM{}'$)}
\label{alg:update_cargo}
\begin{algorithmic}[1]
%
\State $\changedToken{} \gets \emptyset{}$
\Comment{Agents that have changed their token}
%
\For{$\m{h} \in \allM{}$}
\If{$\neg\ \isSinkM{}(\m{h})$}
\label{ln:is_mh_not_a_sink_machine}
\State $\ag{i} = \agentAt{}(\outputCl{}(\m{h}), t+1)$
  \If{$\ag{i} \neq \nullVal{} \wedge \agCl{}(\ag{i}, t) = \tk{0}$}
    \State $\tryToPickup{}(\m{h}, \ag{i}, t, \T{}, \agClM{}, \pkM{}', \changedToken{})$
    \label{ln:ask_ai_to_try_to_pickup_a_token}
  \EndIf
\ElsIf{$\neg\ \isSourceM{}(\m{h})$}
\label{ln:is_mh_not_a_source_machine}
  \State $\ag{i} = \agentAt{}(\inputCl{}(\m{h}), t+1)$
  \If{$\ag{i} \neq \nullVal{} \wedge \agCl{}(\ag{i}, t) \neq \tk{0}$}
  \State $\tryToDeposit{}(\m{h}, \ag{i}, t, T{}, \agTkM{}, \dpM{}', \changedToken{})$
  \label{ln:ask_ai_to_try_to_deposit_a_token}
  \EndIf    
\EndIf
\EndFor
%
\For{$\ag{i} \in \allAg{} - \changedToken{}$}
\label{ln:update_unchanged_tokens_st}
  \State $\agTk{}(\ag{i}, t+1) \gets \agTk{}(\ag{i}, t)$
\EndFor
\label{ln:update_unchanged_tokens_en}
%
\Function{$\tryToPickup{}$}{$\m{h}, \ag{i}, t, \T{}, \agTkM{}, \pkM{}', \changedToken{}$}
\For{$\tk{j} \in \allTk{}$}
\If{$\pk{}'(\m{h}, \T{}, \tk{j}) > 0$}
\label{ln:should_ai_pickup_zj}
  \State $\agTk{}(\ag{i}, t+1) \gets \tk{j}$
  \label{ln:pickup_zj}
  \State $\pk{}'(\m{h}, \T{}, \tk{j}) \gets \pk{}'(\m{h}, \T{}, \tk{j}) - 1$
  \label{ln:adjust_pickup_counter}
  \State $\changedToken{} \gets \changedToken{} \cup \{\ag{i}\}$
  \State \Return{}
\EndIf
\EndFor
\EndFunction
%
\Function{$\tryToDeposit{}$}{$\m{h}, \ag{i}, t, T{}, \agTkM{}, \dpM{}', \changedToken{}$}
\State $\tk{j} \gets \agTk{}(\ag{i}, t)$
\If{$\dpF{}'(\m{h}, \T{}, \tk{j}) > 0$}
\label{ln:ai_has_token_for_mh}
  \State $\agTk{}(\ag{i}, t+1) \gets \tk{0}$
  \label{ln:deposit_token}
  \State $\dpF{}'(\m{h}, \T{}, \tk{j}) \gets \dpF{}'(\m{h}, \T{}, \tk{j}) - 1$
  \label{ln:adjust_deposit_counter}
  \State $\changedToken{} \gets \changedToken{} \cup \{\ag{i}\}$
\EndIf
\EndFunction
\end{algorithmic}
\end{algorithm}

\para{\updateCargo{} (Algorithm~\ref{alg:update_cargo}).} \updateCargo{} updates the token that each agent is carrying. If a machine $\m{h}$'s output cell is occupied by an agent $\ag{i}$ without a token, \updateCargo{} checks if $\ag{i}$ should pick up a token (Lines~\ref{ln:is_mh_not_a_sink_machine}-\ref{ln:ask_ai_to_try_to_pickup_a_token}). Let $\pk{}'(\m{h}, \T{}, \tk{j})$ be the number of additional copies of token $\tk{j}$ that need to be picked up from machine $\m{h}$'s output buffer during epoch $\T{}$. If machine $\m{h}$ has a token $\tk{j}$ which must be picked up (Line~\ref{ln:should_ai_pickup_zj}), \updateCargo{} instructs agent $\ag{i}$ to pick it up (Line~\ref{ln:pickup_zj}) and updates $\pkM{}'$ accordingly (Line~\ref{ln:adjust_pickup_counter}).

Similarly, if machine $\m{h}$'s input cell is occupied by an agent $\ag{i}$ with a token, $\updateCargo{}$ checks if $\ag{i}$ should deposit it (Lines~\ref{ln:is_mh_not_a_source_machine}-\ref{ln:ask_ai_to_try_to_deposit_a_token}). Let $\dpF{}'(\m{h}, \T{}, \tk{j})$ be the number of additional copies of token $\tk{j}$ that need to be deposited in machine $\m{h}$'s input buffer during epoch $\T{}$. If agent $\ag{i}$ is carrying a token $\tk{j}$ that machine $\m{h}$ requires (Line~\ref{ln:ai_has_token_for_mh}), $\updateCargo{}$ deposits it in machine $\m{h}$'s input buffer (Line~\ref{ln:deposit_token}) and updates $\dpM{}'$ accordingly (Line~\ref{ln:adjust_deposit_counter}).

Any agent which does not change the token that it is carrying on timestep $t$ is still carrying the same token on timestep $t+1$ (Lines~\ref{ln:update_unchanged_tokens_st}-\ref{ln:update_unchanged_tokens_en}).

% Move Agents on Road
This function determines how the agents  each agent $\ag{i}$ on the road $\road{h}$. A road cell has a single exit cell. Let $\exit{}(\cl{j})$ be cell $\cl{j}$'s exit cell if $\cl{j}$ is a road cell. If an agent $\ag{i}$ is on a road cell $\cl{j}$ at timestep $t$ and the cell $\exit{}(\cl{j})$ is currently unoccupied at timestep $t+1$, agent $\ag{i}$ is instructed to advance to the cell $\exit{}(\cl{j})$ (Lines~\ref{ln:is_exit_cell_unoccupied}-\ref{ln:agent_ai_moves}). If the cell $\exit{}(\cl{j})$ is occupied at timestep $t+1$, agent $\ag{i}$ is instructed to wait at cell $\cl{j}$ (Line~\ref{ln:agent_ai_waits}).

Let the function $\path{}(\road{i})$ return a list of the cells in road $\road{i}$ starting at its head and ending at its tail. The agents on a road are processed in order of their distance from the road's head (Line~\ref{ln:next_cell_on_road}). Whenever we process an agent $\ag{i}$ on a road, we know if each agent ahead of needs to wait. Consequently, if the cell $\exit{}(\cl{j})$ ahead of agent $\ag{i}$ is unoccupied at timestep $t+1$ when we process $\ag{i}$, we know that no agent ahead of $\ag{i}$ will need to wait on cell $\exit{}(\cl{j})$.


% Flexible Transport System
\para{Flexible Transport System.} A flexible transport system makes it easy to adjust the materials that the machines in a smart factory are supplied with when its manufacturing procedure changes. Most flexible manufacturing systems use a team of agents to transport materials~\cite{AMRs_in_manufacturing_operations}. In traditional smart factories, these agents are autonomous mobile vehicles~\cite{AMRs_in_manufacturing_operations}. In recent mag-lev based manufacturing systems such as BOSCH's ctrlX Flow$^{\text{6D}}$~\cite{BOSCH_maglev} or B\&R Automation's ACOPOS 6D~\cite{BR_maglev}, these agents are mag-lev shuttles. 

% Move Agent on Junction
\para{\moveAgentOnJunction{}.} This function moves agent $\ag{i}$ from junction $\junction{h}$ to one of its exit roads. Let $\tk{j}$ be the token that agent $\ag{i}$ is carrying (Line~\ref{ln:get_ag_token}). Let $\inB{}'(\road{k}, \T{}, \tk{j})$ be the number of additional agents carrying token $\tk{j}$ that need to enter road $\road{k}$ during epoch $\T{}$. Agent $\ag{i}$ is sent to a random exit road $\road{k}$ which needs to receive an additional agent carrying token $\tk{j}$ (Lines~\ref{ln:ln:move_agent_to_exit_road}). 

% PlanForNumEpochs
Each run of \solveTSILP{} has an epoch length $\incrEpochLen{}$ greater than the previous run. Increasing the value of $\incrEpochLen{}$ decreases the runtime of \planForNumEpochs{} but reduces its solution quality. We chose $\incrEpochLen{} = 2$ in our evaluations.


% Cyclic Transport Plan



A cyclic transport plan is associated with an agent permutation $\agP{} : \allAg{} \rightarrow \allAg{}$ and a cycle time $\ct{} \in \mathbb{N}$. It starts and ends at $t=0$ and $t=\ct{}$. The state of an agent $\ag{i} \in \allAg{}$ at $t=0$ is the same as the state of the agent $\Omega{}(\ag{i})$ at $t=\ct{}$.
%
\begin{align*}
    &\forall \ag{i} \in \allAg{}, (\agCl{}(\ag{i},{0}), \agTk{}(\ag{i},0)) = (\agCl{}(\agP{}(\ag{i}), \ct{}), \agTk{}(\agP{}(\ag{i}),\ct{}))
\end{align*}
%
The contents of each buffer at $t{=}0$ and $t=
\ct{}$ are the same.
%
\begin{align*}
    \forall\ \m{i} \in \allM{}, \bIn{}(\m{i},0) = \bIn{}(\m{i},\ct{}) \wedge \bOut{}(\m{i},0) = \bOut{}(\m{i},\ct{}).
\end{align*}
%
A cyclic transport plan can be looped by (a) following its instructions from $t=0$ to $t=
\ct{}$, (b) relabeling each agent  using the agent permutation $\agP{}$ and then (c) repeating.


% Old Alg
\label{ln:make_arrivalT_map}


% Initialize Agents
\begin{algorithm}[t]
\small
\caption{\initializeAgents{}$(\allAg{}, \allTk{}, \allRoads{}, \outBM{}', \pkM{}', \dpM{}')$}
\label{alg:initialize_agents}
\begin{algorithmic}[1]
\State $i \gets 0$
\For{$\road{h} \in \allRoads{}$}
  \State $\nextEmptyCell{} \gets \head{}(\road{h})$
  \For{$\tk{j} \in \allTk{} \cup \{\tk{0}\}$}
    \While{$\outB{}(\road{h}, \tk{h}, 0) > 0$}
      \State $\at{}(\nextEmptyCell{}, 0) \gets \ag{i}$
      \State $\agTk{}(\ag{i}, 0) \gets \tk{j}$
      \State $\nextEmptyCell{} \gets \next{}(\nextEmptyCell{})$
      \State $i \gets i + 1$
    \EndWhile
  \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}

% Very old TS-ACES text


\para{\TSACES{}.} \TSACES{} generates traffic system embeddings using the traffic system planner $\tsPlanner{}$ (Line~\ref{ln:get_traffic_system_based_embedding}). It then converts them into a cell based embedding as follows. 

First, \TSACES{} initializes the matrices that it will use to store the state of its agents. \TSACES{} stores agent positions in a $|\allCl{}| \times \numEpochs{} \cdot \epochLen{}$ occupancy matrix $\atM{}$ (Line~\ref{ln:make_occupancy_matrix}). The field $\at{}(\cl{h}, t)$ stores the agent $\ag{i}$ which occupies cell $\cl{h}$ at timestep $t$. If cell $\cl{h}$ is unoccupied on timestep $t$, $\at{}(\cl{h},t) = \nullVal{}$. \TSACES{} stores the cargo that each agent is carrying on each timestep $t$ in a cargo matrix $\agTkM{}$ (Line~\ref{ln:make_cargo_matrix}). Initially, no cell is assigned an agent and no agent is assigned a token on any timestep $t$.

% Old TS-ACES text
\para{\TSACES{}.} \TSACES{} stores agent positions in a $|\allCl{}| \times \numEpochs{} \cdot \epochLen{}$ occupancy matrix $\atM{}$ (Line~\ref{ln:make_occupancy_matrix}). The field $\at{}(\cl{h}, t)$ stores the agent $\ag{i}$ that occupies cell $\cl{h}$ at timestep $t$. If cell $\cl{h}$ is unoccupied on timestep $t$, $\at{}(\cl{h},t) = \nullVal{}$. It stores its agents' cargo in a cargo matrix $\agTkM{}$ (Line~\ref{ln:make_cargo_matrix}). The epoch at which each agent entered its current road is stored in the map $\arrivalT{} : \allAg{} \rightarrow \mathbb{Z} \cup \{\nullVal{}\}$ (Line~\ref{ln:make_arrivalT_map}). Tracking this information prevents agents from advancing two roads in one epoch.

% Old Gen Buffer Contents
\para{\genBufferContents{}.} We initialize each machine's input buffer with every token that it consumes in a single cycle. Since every one of these tokens will be replaced by the start of the next cycle, a machine will never run out of tokens and stall. We initialize each machine's output buffer with every token that it emits in a single cycle for similar reasons. Once we know which machines are in a buffer on timestep $t=0$, we can use the pickup $\pkM{}$ and deposit $\dpM{}$ tensors to compute its contents on every other timestep.

%
% After finding its agents' states on every timestep, \TSACES{}:
% %
% \begin{enumerate}
%     \setcounter{enumi}{3}
    
%     \item Converts its occupancy matrix $\atM{}$ into the position matrix $\agClM{}$ (Lines~\ref{ln:iterate_over_timesteps}-\ref{ln:convert_atF_to_posF}).

%     \item Computes the state of every buffer at every timestep 
% \end{enumerate}

% Old Traffic System Based Embedding Text
A traffic system based embedding's transport plan is based on roads rather than individual cells. It aggregates timesteps into epochs. The epoch length parameter $\epochLen{}$ specifies the number of timesteps in an epoch. At the start of each epoch, each agent is queued at the head of some road. Each epoch, every agent must pass through the junction at the end of its current road and join a queue at the head of one of the junction's exit roads. 

A traffic system based embedding treats agents carrying the same token as indistinguishable. It divides agents into $|\allTk{} + 1|$ classes, one class for every type of token. When an agent picks up or deposits a token, it changes classes.

A smart factory often has to run a manufacturing procedure for an indefinite length of time. We would therefore like to construct a cyclic transport plan, a transport plan which can be looped an arbitrary number of timesteps~\cite{CCPP}. We associate our traffic system based transport plan is with a number of epochs $\numEpochs{}$. It loops after running for $\numEpochs{}$ epochs. 



Our embedding loops after $\numEpochs{}$ epochs. Consequently, its values for epoch $\T{} = 0$ and epoch $\T{} = \numEpochs{}$ are the same. For example:
%
\begin{align*}
\forall\ \road{i} \in \allRoads{},\ \T{} \in [0.&.\numEpochs{}],\ \forall\ \tk{j} \in \allTk{} \cup \{\tk{0}\},\\
%
&\inB{}(\road{i}, 0, \tk{j}) = \inB{}(\road{i}, \T{}, \tk{j}).
\end{align*}
%
Analogous statements exist for $\outBM{}$, $\pkM{}$ and $\dpM{}$.

% Old Conversion Algorithm




%Initially, no agent occupies a cell or carries a token on any timestep $t$.

$\TSTGEN{}$ determines the  state $\sfState{}(0)$ of the smart factory at timestep $0$ using the function $\initializeSF{}$. It computes the state $\sfState{}(t+1)$ of the smart factory on timestep $t+1$ by:
%
\begin{enumerate}
    % \item Generating an occupancy vector $\atM{}(t)$ using the function $\genOccupancyVec{}(\agClM{}(t))$ (Line~\ref{}).

    \item Moving each agent on a junction at timestep $t$ using the function $\moveAgentOnJunction{}$ (Lines~\ref{ln:iterate_over_junctions}-\ref{ln:move_agent_on_junction}).

     \item Moving each agent on a road at timestep $t$ using the function $\moveAgentsOnRoad{}$ (Lines~\ref{ln:iterate_over_roads}-\ref{ln:move_agents_on_road}).
     
     \item Computing the cargo that each agents carry at timestep $t+1$ using the functions $\depositToken{}$ (Line~\ref{ln:deposit_token}), $\pickupToken{}$ (Line~\ref{ln:pickup_token}) and $\keepToken{}$ (Line~\ref{ln:keep_token}).

     % \item Computing the state of every buffer using the function $\genBufferContents{}$ (Line~\ref{ln:gen_buffer_contents}).
\end{enumerate}
%
%
We now describe each of $\TSTGEN{}$' functions in detail.

% Old move agents on junction
\para{\moveAgentOnJunction{}. (Lines~\ref{ln:move_agent_on_junction_begin}-\ref{ln:update_arrivalT})} This function moves an agent $\ag{i}$ on a junction $\junction{h}$ to one of the junction's exit roads. Let $\tk{j} \in \allTk{} \cup \{\tk{0}\}$ be the token that agent $\ag{i}$ is carrying. Let $\inB{}'(\road{k}, \T{}, \tk{j})$ be the number of additional agents carrying token $\tk{j}$ that need to enter road $\road{k}$ during epoch $\T{}$.  Agent $\ag{i}$ is moved to the tail $\tail{}(\road{k})$ of some road $\road{k}$ which needs to receive an extra agent carrying token $\tk{j}$. The value of $\arrivalT{}(\ag{i})$ is then updated accordingly. 

% Old Move Agents on Road
\para{\moveAgentsOnRoad{} (Algorithm~\ref{alg:move_agent_on_road}).} This function determines how the agents on road $\road{h}$ move. Let $\exit{}(\cl{j})$ be cell $\cl{j}$'s exit cell if cell $\cl{j}$ is a road cell. Let $\exit{}(\cl{j})$ be undefined otherwise. If agent $\ag{i}$ is at the head of road $\road{h}$ and it entered road $\road{h}$ during the current epoch $\T{}$, it waits on cell $\cl{j}$ (Line~\ref{ln:arrived_with_epoch_check}-\ref{ln:agent_ai_waits_to_avoid_double_advance}). Otherwise, if $\ag{i}$ is on the cell $\cl{j}$ at timestep $t$ and the cell $\exit{}(\cl{j})$ is not currently occupied on timestep $t+1$ (Lines~\ref{ln:is_exit_cell_unoccupied}), it  moves to the cell $\exit{}(\cl{j})$ (Line~\ref{ln:agent_ai_moves}). Otherwise, agent $\ag{i}$ waits on cell $\cl{j}$ (Line~\ref{ln:agent_ai_waits}).

% Old deposit tokens
\para{\depositToken{} (Algorithm~\ref{alg:deposit_token}).} If a machine $\m{h}$'s input cell $\inputCl{}(\m{h})$ is occupied by an agent $\ag{i}$ carrying a non-null token $\tk{j}$, $\depositToken{}$ checks if $\ag{i}$ should deposit $\tk{j}$ into $\m{h}$'s input buffer.  Let $\dpF{}'(\m{h}, \arrivalT{}(\ag{i}), \tk{j})$ be the number of additional copies of token $\tk{j}$ that need to be deposited into $\m{h}$'s input buffer by agents which entered road $\road{h}$ during epoch $\arrivalT{}(\ag{i})$. If $\dpF'(\m{h}, \arrivalT{}(\ag{i}), \tk{j}) > 0$ (Line~\ref{ln:ai_has_token_for_mh}), agent $\ag{i}$'s cargo on timestep $t+1$ is the null token $\tk{0}$ (Line~\ref{ln:deposit_token_instr}) and a copy of token $\tk{j}$ is added to the contents $\bIn{}(\m{h}, t+1)$ of $\m{h}$'s input buffer (Line~\ref{ln:adjust_input buffer}).

% Old Pickup Tokens
If a machine $\m{h}$'s output cell is occupied by an agent $\ag{i}$ without a (non-null) token, \pickupToken{} checks if $\ag{i}$ should pick up a token from $\m{h}$'s output buffer. \pickupToken{} works analogously to \depositToken{}.
